Endo-Sim2Real: Consistency learning-based domain adaptation for instrument segmentation

Surgical tool segmentation in endoscopic videos is an important component of computer assisted interventions systems. Recent success of image-based solutions using fully-supervised deep learning approaches can be attributed to the collection of big labeled datasets. However, the annotation of a big dataset of real videos can be prohibitively expensive and time consuming. Computer simulations could alleviate the manual labeling problem, however, models trained on simulated data do not generalize to real data. This work proposes a consistency-based framework for joint learning of simulated and real (unlabeled) endoscopic data to bridge this performance generalization issue. Empirical results on two data sets (15 videos of the Cholec80 and EndoVis'15 dataset) highlight the effectiveness of the proposed \emph{Endo-Sim2Real} method for instrument segmentation. We compare the segmentation of the proposed approach with state-of-the-art solutions and show that our method improves segmentation both in terms of quality and quantity.

==> Tables/Clean.tex <==
%\begin{document}

\begin{tabular}{|l|c c c c|}
    \hline
          & $Our_{Sim\rightarrow X}$ & $Our_{SimCholec\rightarrow X}$ & $I2I_{SimCholec\rightarrow X}$ & $FS_{Real_{UL}\rightarrow X}$ \\
        \hline
        \hline
        %{\tiny{Hook}} & \parbox[c][1.5cm]{2.37cm}{\includegraphics[width=2.37cm, height=1.35cm]{video76_frame_36000_mask.jpg}} & \parbox[c][1.5cm]{2.37cm}{\includegraphics[width=2.37cm, height=1.35cm]{01_Sim2Random.jpg}} & \parbox[c][1.5cm]{2.37cm}{\includegraphics[width=2.37cm, height=1.35cm]{01_Sim2Cholec.jpg}} & \parbox[c][1.5cm]{2.37cm}{\includegraphics[width=2.37cm, height=1.35cm]{01_Cholec.jpg}} \\
        %\hline
        {\tiny{Grasper \&  Hook }} & \parbox[c][1.5cm]{2.37cm}{\includegraphics[width=2.37cm, height=1.35cm]{video72_frame_01750_mask.jpg}} & \parbox[c][1.5cm]{2.37cm}{\includegraphics[width=2.37cm, height=1.35cm]{02_Sim2Random.jpg}} & \parbox[c][1.5cm]{2.37cm}{\includegraphics[width=2.37cm, height=1.35cm]{02_Sim2Cholec.jpg}} & \parbox[c][1.5cm]{2.37cm}{\includegraphics[width=2.37cm, height=1.35cm]{02_Cholec.jpg}} \\
        \hline 
        {\tiny{Bipolar}} & \parbox[c][1.5cm]{2.37cm}{\includegraphics[width=2.37cm, height=1.35cm]{video74_frame_16000_mask.jpg}} & \parbox[c][1.5cm]{2.37cm}{\includegraphics[width=2.37cm, height=1.35cm]{03_Sim2Random.jpg}} & \parbox[c][1.5cm]{2.37cm}{\includegraphics[width=2.37cm, height=1.35cm]{03_Sim2Cholec.jpg}} & \parbox[c][1.5cm]{2.37cm}{\includegraphics[width=2.37cm, height=1.35cm]{03_Cholec.jpg}} \\
        \hline 
        {\tiny{Clipper}} & \parbox[c][1.5cm]{2.37cm}{\includegraphics[width=2.37cm, height=1.35cm]{video76_frame_21500_mask.jpg}} & \parbox[c][1.5cm]{2.37cm}{\includegraphics[width=2.37cm, height=1.35cm]{06_Sim2Random.jpg}} & \parbox[c][1.5cm]{2.37cm}{\includegraphics[width=2.37cm, height=1.35cm]{04_Sim2Cholec.jpg}} & \parbox[c][1.5cm]{2.37cm}{\includegraphics[width=2.37cm, height=1.35cm]{04_Cholec.jpg}} \\
        \hline 
        {\tiny{Scissors}} & \parbox[c][1.5cm]{2.37cm}{\includegraphics[width=2.37cm, height=1.35cm]{video76_frame_35125_mask.jpg}} & \parbox[c][1.5cm]{2.37cm}{\includegraphics[width=2.37cm, height=1.35cm]{05_Sim2Random.jpg}} & \parbox[c][1.5cm]{2.37cm}{\includegraphics[width=2.37cm, height=1.35cm]{05_Sim2Cholec.jpg}} & \parbox[c][1.5cm]{2.37cm}{\includegraphics[width=2.37cm, height=1.35cm]{05_Cholec.jpg}} \\
        \hline 
        {\tiny{Irrigator}} & \parbox[c][1.5cm]{2.37cm}{\includegraphics[width=2.37cm, height=1.35cm]{video74_frame_21500_mask.jpg}} & \parbox[c][1.5cm]{2.37cm}{\includegraphics[width=2.37cm, height=1.35cm]{04_Sim2Random.jpg}} & \parbox[c][1.5cm]{2.37cm}{\includegraphics[width=2.37cm, height=1.35cm]{06_Sim2Cholec.jpg}} & \parbox[c][1.5cm]{2.37cm}{\includegraphics[width=2.37cm, height=1.35cm]{06_Cholec.jpg}} \\
        \hline
\end{tabular}

%\end{document}

==> Tables/Quants.tex <==
\begingroup
\begin{tabular}   % top level tables, with 2 rows
    \centering
	\setlength{\tabcolsep}{10pt} % Default value: 6pt
    \renewcommand{\arraystretch}{1.2} % Default value: 1
    Comparison-$I2I$ & Comparison-$CL$ \\  
    % bottom left of the top level table: table 1 
    \begin{minipage}[t]{.4\textwidth}
    \centering
    \vspace{0pt}
    \begin{tabular}{| l | c | c |}
		\hline
		Method & $SR\rightarrow Real_L$ & $SC\rightarrow Real_L$ \\
		\hline 
		\hline
		I2I & .75 & .77 \\ 
		Ours & \textbf{.81} & \textbf{.80} \\ 
		\hline
	\end{tabular}
	\end{minipage}
	  % starting bottom right of the top level table
    % table 2
    \begin{minipage}[t]{.6\textwidth}
    \centering
    \vspace{0pt}
    \begin{tabular}{| l | c |}
    	\hline
    	Method & $Sim\rightarrow Real_L$ \\
    	\hline 
    	\hline
    	Pi-Model & .62 \\ 
    	Ours & \textbf{.75} \\
    	\hline
    \end{tabular}
    \end{minipage} \hfill
\end{tabular}
\endgroup
